SoK: Systematization and Benchmarking of Deepfake Detectors in a Unified Framework

Deepfakes have rapidly emerged as a serious threat to society due to their ease of creation and dissemination, triggering the accelerated development of detection technologies. However, many existing detectors rely on labgenerated datasets for validation, which may not prepare them for novel, real-world deepfakes. This paper extensively reviews and analyzes state-of-the-art deepfake detectors, evaluating them against several critical criteria. These criteria categorize detectors into 4 high-level groups and 13 finegrained sub-groups, aligned with a unified conceptual framework we propose. This classification offers practical insights into the factors affecting detector efficacy. We evaluate the generalizability of 16 leading detectors across comprehensive attack scenarios, including black-box, white-box, and graybox settings. Our systematized analysis and experiments provide a deeper understanding of deepfake detectors and their generalizability, paving the way for future research and the development of more proactive defenses against deepfakes.

==> Sections/3_method.tex <==
\section{Methodology}
\label{sec:methodology}
\sha{I like this section as it sets the story. But one reviewer said it is made redundant by other sections. So either we significantly reduce the size of this section or remove it entirely. I am thinking about option 1 for now but we might have to go with option 2 to save space. After thought maybe we could use option 3. which is to move each of the subsections in this section as a overview to that section where appropriate and therefore we could remove redundancy in those sections as well.}
\textcolor{gray}{This section details our methodology for obtaining answers to our main research questions.}

\textcolor{gray}{\subsection{Methodology for RQ1} To address the first research question, we conducted a systematization of the existing literature on deepfake detectors. To do this, we followed a stringent process with the objective to identify the key influential factors in facial deepfake detection. The process began with the meticulous collection of research papers related to deepfake detection. We describe the entire process, encompassing the inclusion and exclusion criteria for selecting these papers, in Sec.~\ref{sub:PaperSelectionCriteria}. This process produced {51} relevant papers. Subsequently, each of these {51} articles were systematically reviewed, considering factors such as dataset utilization, methodology focus, pre-processing methods, model architecture, and model evaluation criteria (see Sec. \ref{sub:DetectorsAnalysis}). After decomposing the methodologies of individual deepfake detectors, we collated their information to construct a conceptual framework providing a holistic view of the detection process. This conceptual framework facilitates the systematization of the existing literature, mapping each method to its place in the conceptual framework. We further categorize the detectors using this conceptual framework based on the focus of their methodology into 4 high-level groups and 13 fine-grained sub-groups,  providing more  clarity  to our systematization. The complete process is expounded on in Sec. \ref{sec:method}. Finally, we present the influential factors derived from this exercise in Sec. \ref{sub:inpact_factors}.}

\textcolor{gray}{\subsection{Methodology for RQ2} To address the second research question, we systematically evaluated the performance of deepfake detectors on various deepfake datasets to ensure a rigorous and equitable comparison. We started this process by meticulously selecting a subset of detectors from those previously identified in \textit{\textbf{RQ1}}, employing stringent inclusion and exclusion criteria, as detailed in Sec.~\ref{sec:DetectorforEvaluation}. 
This careful curation yielded {16} detectors, forming the basis for our subsequent generalization experiments. To facilitate this evaluation, the subsequent step involved the selection of appropriate evaluation strategies and datasets for experimentation. We selected, collected, and generated deepfake datasets encompassing three distinct evaluation settings: gray-box, white-box, and black-box (see Sec.~\ref{sec:Evaluation Strategies} and \ref{sub:dataset_evaluation}). Finally, the results of our detector generalizability experiments are presented and analyzed in Sec.~\ref{sec:experiments}.}

\textcolor{gray}{\subsection{Methodology for RQ3} To answer the third research question, in Sec.~\ref{sub:inpact_factors}, we take the generalizability results from gray-box, white-box, and black-box settings and analyze them using the lens of the conceptual framework and the influential factors identified in \textit{\textbf{RQ1}} in Sec~\ref{sec:experiments}. Based on this analysis, we provide our insights and recommendations in Sec.~\ref{sub:inpact_factors} as well as discuss the gaps in the literature and provide directions for future research in Sec.~\ref{sec:limit}.}

